MimicPlay: Long-Horizon Imitation Learning by Watching Human Play

Imitation learning from human demonstrations is a promising paradigm for teaching robots manipulation skills in the real world. However, learning complex long-horizon tasks often requires an unattainable amount of demonstrations. To reduce the high data requirement, we resort to human play data - video sequences of people freely interacting with the environment using their hands. Even with different morphologies, we hypothesize that human play data contain rich and salient information about physical interactions that can readily facilitate robot policy learning. Motivated by this, we introduce a hierarchical learning framework named MimicPlay that learns latent plans from human play data to guide low-level visuomotor control trained on a small number of teleoperated demonstrations. With systematic evaluations of 14 long-horizon manipulation tasks in the real world, we show that MimicPlay outperforms state-of-the-art imitation learning methods in task success rate, generalization ability, and robustness to disturbances. Code and videos are available at https://mimic-play.github.io

==> table6_tasks.tex <==
\begin{table*}
    \centering
    \begin{tabular}{c|c|m{11cm}}
    \toprule
     \multirow{3}{*}[-20pt]{Kitchen}   & Task-1 
      & \begin{itemize}
      \item Initial state: A drawer is placed on the left side of the table. The drawer is not fully open and contains pumpkin and lettuce. A closed microwave oven is placed on the right side of the desktop. A bowl and a stove are placed on the lower edge of the tabletop. There is a carrot inside the bowl. A pan is placed on top of the stove. 
      \item Subgoals: a) Open the microwave oven door. b) Pull out the microwave oven tray. c) Pick up the bowl. d) Place the bowl on the microwave tray.
      \end{itemize} \\
      \cline{2-3}
        & Task-2 & \begin{itemize}
        \item Initial state: same as Kitchen Task-1.
        \item Subgoals: a) Open the drawer.
            b) Pick up the carrot.
            c) Put the carrots in the drawer.
        \end{itemize} \\
        \cline{2-3}
        & Task-3 & \begin{itemize}
        \item Initial state: same as Kitchen Task-1.
        \item Subgoals: a) Pick up the pan.
            b) Place the pan on the table.
            c) Pick up the bowl.
            d) Place the bowl on the stove.
        \end{itemize} \\
        \midrule
        \multirow{7}{*}[-70pt]{Study desk} & Task-1 &
    \begin{itemize}
        \item Initial state: The book is on the rack. The lamp is on. The box is opened and closed in a random state. The pen is located either in the center of the table or in the box.
        \item Subgoals: a) Turn off the lamps. b) Pick up the book. c) Place the book on the shelf position.
    \end{itemize} \\
    \cline{2-3}
    & Task-2 &
    \begin{itemize}
        \item Initial state: The location of the book is either on the shelf or on the rack. The lamp is off. The box is closed. The pen is in the center of the table.
        \item Subgoals: a) Turn on the lamps.
b) Open the box. c) Pick up the pen. d) Put it in the box.
    \end{itemize}\\
    \cline{2-3}
    & Task-3 &
    \begin{itemize}
        \item Initial state: The book is on the rack. The state of the lamp is random. The box is closed. The pen is in the center of the table.
        \item Subgoal a) Open the box.
            b) Pick up the pen.
            c) Place the pen in the box.
            d) Pick up the book.
            e) Place the book on the shelf.
        \end{itemize}\\
        \cline{2-3}
    & Task-4 & 
    \begin{itemize}
        \item Initial state: The location of the book is either on the shelf or on the rack. The lamp is on. The box is closed. The pen is located either in the center of the table or in the box.
        \item Subgoals: a) Open the box.
            b) Turn off the lamp.
        \end{itemize}\\
    \bottomrule
    \end{tabular}
    \caption{Task definition 1.}
    \label{tab:details_of_the_goals_of_each_task}
\end{table*}


\begin{table*}
    \centering
    \begin{tabular}{c|c|m{11cm}}
    \toprule
    \multirow{3}{*}[-70pt]{Study desk} 
    & Easy & 
    \begin{itemize}
        \item Initial state: The location of the book is either on the shelf or on the rack. The lamp is off. The box is closed. The pen is located either in the center of the table or in the box.
        \item Subgoals: a) Turn on the lamp.
            b) Open the box.
            c) Turn off the lamp.
        \end{itemize}\\
        \cline{2-3}
    & Medium & 
    \begin{itemize}
        \item Initial state: The location of the book is either on the shelf or on the rack. The lamp is on. The box is closed. The pen is in the center of the table.
        \item Subgoals: a) Open the box. b) Turn off the lamp. c) Pick up the pen. d) Place the pen in the box.
        \end{itemize}\\
        \cline{2-3}
    & Hard & 
    \begin{itemize}
        \item Initial state: The book is on the shelf. The lamp is on. The box is closed. The pen is located either in the center of the table or in the box.
        \item Subgoals: a) Turn off the lamp.
            b) Open the box.
            c) Pick up the book.
            d) Place the book on the shelf.
        \end{itemize}\\
    \midrule
    Flower & - &  
    \begin{itemize}
    \item Initial state: Two flowers and a vase are placed on the table. The vase will randomly be placed on the top left or top right corner of the table.
    \item Subgoals: a) Picking up a flower.
        b) Insert the flower into the vase.
        c) Pick up the other flower.
        d) Insert the flower into the vase.
    \end{itemize}\\
    \midrule
     Whiteboard & - & 
    \begin{itemize}
    \item Initial state:
    A whiteboard and board eraser are placed on the table. The board eraser is placed on the left side of the whiteboard.
    \item Subgoals: a) Pick up the board eraser.
        b) Moves over the curve line.
        c) Erase the curve line.
        d) Return the eraser to the original location.
    \end{itemize}\\
    \midrule
    Sandwich & - & 
    \begin{itemize}
    \item Initial state: A circular ingredient selector is placed in the upper right corner of the table. Half of the circle holds ingredients for a sandwich (bread, lettuce, sliced tomato) and half holds ingredients for a cheeseburger (bread, cheese, burger patty). A white plate is placed in the lower left corner of the table.
    \item Subgoals for a sandwich:
        a) Rotate the ingredient selector to the right position. Pick up a piece of bread from it and place it on the plate.
        b) Rotate the ingredient selector to the correct position. Pick up the lettuce and place it on top of the bread.
        c) Rotate the ingredient selector to the right position. Pick up the sliced tomato and place it on top of the lettuce.
        d) Rotate the ingredient selector to the right position. Pick up another piece of bread and place it on top of the tomato.
    \end{itemize}\\
    \midrule
    Cloth & - & 
    \begin{itemize}
    \item Initial state: An unfolded brown cloth is randomly placed on the table. 
    \item Subgoals: a) The robot folds the cloth in half once to become 1/2 of its original size. b) The robot folds the cloth once more to become 1/4 of its original size.
    \end{itemize}
        \\
    \bottomrule
    \end{tabular}
    \caption{Task definition 2.}
    \label{tab:details_of_the_goals_of_each_task_2}
\end{table*}
